Venn GAN: Discovering Commonalities and Particularities of Multiple Distributions

We propose a GAN design which models multiple distributions effectively and discovers their commonalities and particularities. Each data distribution is modeled with a mixture of $K$ generator distributions. As the generators are partially shared between the modeling of different true data distributions, shared ones captures the commonality of the distributions, while non-shared ones capture unique aspects of them. We show the effectiveness of our method on various datasets (MNIST, Fashion MNIST, CIFAR-10, Omniglot, CelebA) with compelling results.

==> misc.tex <==






\begin{itemize}
	\item GAN operates on single distribution. There might be multiple distribution to model where the distributions have unique supports and common supports. This paper is the first step to model multiple distributions to discover their intersections an uniqueness.
    \item Show the toy example where each region emits only a single value. Show that the constructed model has unique solution. 
of each mode of the generator. One interpretation of a generator with n modes is n generator with tied weights (parameter
sharing). How to call individual/unique/novel and common/intersection modes?
\item Given enough capacity individual modes can generate all other modes. This happens when the frequency of lower
intersections overwhelm higher intersections. If the modes are equally likely or higher intersections are more common
than the lower ones, then leaking does not occur as higher intersection mode can not generate lower intersections.
\item Theories about optimality similar to original GAN paper. For example, if the model is stable at convergence or behavior
of non-adversarial part etc.
\end{itemize}

What are the experiment we have right now?
Mnist          ( diff frequency/ more than one class modes / 2-3 sets)
Mnist fashion  ( diff frequency/ more than one class modes / 2-3 sets)
cifar10        ( diff frequency/ more than one class modes / 2-3 sets)
omniglot       (       -       /            -              / 2-3 sets) (4 or more sets?)
coMNIST        (       -       /            -              / 2   sets) (may not be necessary. Maybe for appendix)

Not modeled yet:
CelebA-males/females, Dogs/Cats , modeling of region-8


\begin{itemize}
    \item What are the drawback and how we did deal with them.
    \item Type of experiments we can do with it.
\end{itemize}

$\alpha$ values represent how much to sample from each regions as each regions contribution to the union can vary. When the method is interpreted in probabilistic way, normalized $\alpha$ values corresponds to priors or contributions similar to Gaussian Mixture Model. In this work we have treated $\alpha$ values as hyper-parameters by simplifying them which is regions with same interaction type share the same $\alpha$ e.g. $\alpha_1$ = $\alpha_2$ = $\alpha_3$, $\alpha_4$ = $\alpha_5$ = $\alpha_6$. This simplification reduces number of hyper parameters to $n-1$ for $n$ distribution game when $\alpha$ value for $n$-way intersection kept constant.


The method described above, converges to satisfactory results on various datasets when $\alpha$ values are properly tuned. However this is not an easy task as we don't know what should be the contributions of regions to model true data distributions correctly. When contributions of regions does not roughly match with true data distributions, then commonality loss can be overwhelmed and leaking occurs between the regions (See \ref{ref to experiment} for experimental results of this phenomena). We have encountered two types of leaking issue. In the first type low intersection regions includes some portion of high intersection regions such as 2,3-way intersection to no-intersection or 3-way intersection to 2-way intersection. This happens when contribution of low intersection regions are higher than what it should be in true data distribution. That leads low intersection regions to help other regions in the union by taking some portions of them. The second type is reverse of the previous situation namely high-intersection regions represents some part of low-intersection regions. This happens when consensus loss is overwhelmed by large contribution of high intersection regions which does not match to its correspondence in true data distribution. In order to alleviate this issue we included an additional objective which aims to separate regions, one from another:

\begin{equation}
\max_{\theta,\phi_c} E_{z \sim p_{z}(\boldsymbol z)} \log C(y_i | \boldsymbol r_i ; \phi_c) = E_{z \sim p_{z}(\boldsymbol z)} \log C(y_i | G(z,c=i ; \theta) ; \phi_c)
\label{classification_formulation}
\end{equation}

where $y_i$ is one-hot label for $\boldsymbol r_i$ and $C$ is a classifier which outputs probability distribution over regions. With this objective classifier tries to separate regions and generator tries to place its regions at the positive side of the separation hyperplane. This objective enforces separation of regions at a toll of mimicking each true data distribution. Similar losses has been used by \citet{hoang2018mgan} previously. Combined objective becomes:

\begin{equation}
\min_{G,C} \max_{D_1,D_2, ..., D_n} V(D_1,D_2, ..., D_n,G) - \lambda E_{z \sim p_{z}(\boldsymbol z)} \log C(y_i | G(z,c=i ; \theta) ; \phi_c)
\label{overall_equation}
\end{equation}

where $\lambda$ is balancing hyper-parameter between the two terms.

\begin{itemize}
    \item 2 agents and 3 agents experiments. Distributions with more than one object class in each region to show robustness. Multiple modes in each region (Vijay).
    \item Some analysis on leaking problem. How changing prior (contribution) of each mode deals with leaking problem.
    \item Does it work better than cGAN (CS)?
    \item Interpolation between the modes. It aims to visualize how latent space of the generator modeled by passing through one region of venn to another. Expectation: Meaningful change between the modes.
    \item Ablation study 1: NEW IDEAS ARE NEEDED HERE, what type of experiments we can conduct to show the behavior of the method?
    \item Ablation study 2: Question: Why the modes correlate with classes but not styles (referring to mnist, mnist fashion etc)? Hypothesis: The major variation in the datasets is change of digits not style. Maybe we can show this with eigen-vector analysis on mnist, mnist-fashion. It would be nice to show that there are cases where it correlates with style but not object type (colored mnist can help?).
    \item More results with natural datasets like omniglot, celeba, dogs and cats datasets 
    \item Application 1: Multi-task learning where set1 is small amount of images while set2 contains large amount. Set1 is considered as subset of Set2. Can we improved the performance of Set1? How performance changes with different number of samples from Set1. Use both visual and FID metric to show performance. 
    \item Application 2: Semi-supervised learning (Bruno)
    \item VennGAN for assessment of separately trained generative model. (Bruno)
    \item VennGAN to improve a generative model by finding its missing modes and improving through combination. Try it on CIFAR10?  
\end{itemize}

May call v1, v2 as type I, type II etc.
Training distributions by independence assumption. It might show as difference as the generator is shared.
*** Distributions are not denoted correctly. Use D instead of p(x) ***

Application: recovering a distribution with v2 type? Imagine a scenario where we have samples from a distribution but the set is corrupted with samples from another distribtuion.



\begin{equation}
 \boldsymbol{p_{data}} = \boldsymbol{O} \boldsymbol{p_g}
\end{equation}

\textbf{One type of explanation:} Each region in the venn diagram is going to be associated with a generator whose implicit distribution should be equal to the true distribution of the region. 

OR true data distributions are mixture of distributions:

\begin{equation}
\begin{aligned}
    p_{data_i} (\boldsymbol{x})= \sum_{j=1}^n o_j p_{r_j} \\
\end{aligned}
\end{equation}

%\begin{equation}
%V(D_1,D_2, ..., D_n,G) = \sum_{i=1}^n E_{x \sim p_{data_i}(\boldsymbol x)}[log D_i(\boldsymbol x ; \phi_i)] + E_{u \sim p_{i}(\boldsymbol u)}[log(1-D_i(\boldsymbol u ; \phi_i))]
%\label{venn_gan_formulation}
%\end{equation}

%\begin{equation}
%p_{i}(\boldsymbol u) = p_{S_i}(\boldsymbol x) = \frac{1}{\left\vert{S_i}\right\vert} \sum_{r \in S_i} p_{G_r}(\boldsymbol x)
%\label{union_formulation}
%\end{equation}

%where $p_{i}(\boldsymbol x)$ is $i$-th true data distribution and $p_{i}(\boldsymbol u)$ is $i$-th generated distribution which tries to mimic $p_{i}(\boldsymbol x)$.

\comment{
\begin{equation}\label{eq:matrixeqn}
\begin{aligned}

    \begin{bmatrix}
        p_{data_1} \\
        p_{data_2} \\
        \vdots \\
        p_{data_n}
    \end{bmatrix}
    &=
    \begin{bmatrix}
        1 & 0 & \cdots & 0 \\
        0 & 1 & \cdots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        0 & 0 & \cdots & 1
    \end{bmatrix}
    \begin{bmatrix}
        p_{g_1} \\
        p_{g_2} \\
        \vdots \\
        p_{g_n}
    \end{bmatrix}
\end{aligned}
\end{equation}
}

%As shown in the theorem ..., at global minimum of $C(G)$ is:
By following Theorem 1 of \cite{gan} for each discriminator, we can show that:

\begin{equation}
\begin{aligned}
    p_{data_i}(\boldsymbol x) &=p_{g_i}(\boldsymbol x) \\
    &= \frac{1}{|S_i|} \sum_{r_j \in S_i} p_{r_j}
\end{aligned}
\end{equation}

*** Can we pull out $p_{r_j}$ and show what they capture? Maybe some toy examples( mixture of gaussians in analytic form) to show how each $p_{r_j}$ captures the right gaussian distribution.***

In order to successfully represent Venn Diagram like interactions there should be constraints on the regions:
\begin{itemize}
    \item Restriction 1: Combination of all regions that belong to the same set should be equal to distribution of that set i.e. $Supp(p_{data_i}) = \sum_{r_j \in S_i} Supp(p_{r_j})$.
    \item Restriction 2: Each region represents a different part of the distribution i.e. $Supp(p_{r_j}) \cap Supp(p_{r_k}) = \left\{ \right\} \forall r_j, r_k \in S_i$. 
    \item Restriction 3: Regions with intersections should belong to all corresponding distributions.
    \item By satisfying Restriction 1 and 2, individual regions represent unique parts of the corresponding distributions.
\end{itemize}

\comment{
\begin{figure}[h!]
	\centering
	\includegraphics[width=1.0\linewidth]{gan_vs_vengann.pdf}
	\caption{Illustration of difference between GAN and VennGAN. GAN models single distribution while VennGAN models multiple distributions with their interactions}
	\label{gan_vs_vengann}
\end{figure}
}

GAN learns to model a single distribution. Expending it to multiple distribution can be achieved by training $n$ GAN models in parallel for $n$ distributions. However this naive implementation would omit potential interactions between the distributions. The distributions interaction might come in different forms.

\begin{equation}
\min_{G} \max_{D_1,D_2, ..., D_n} V(D_1,D_2, ..., D_n,G)
\label{multi_agent_gan_formulation}
\end{equation}

\begin{equation}
\begin{split}
    V(D_1,D_2, ..., D_n,G) = \\
    \frac{1}{n}\sum_{i=1}^n E_{x \sim p_{data_i}(\boldsymbol x)}[log D_i(\boldsymbol x)] + \\
    \frac{1}{n}\sum_{i=1}^n E_{x \sim p_{g_i}(\boldsymbol x)}[log(1-D_i(\boldsymbol x))]
\label{venn_gan_formulation}
\end{split}
\end{equation}

\begin{equation}
    p_{g_i}(\boldsymbol x) = \frac{1}{|S_i|} \sum_{r_j \in S_i} p_{r_j}
\end{equation}

where $p_{data_i}(\boldsymbol x)$ is $i$-th true data distribution, $p_{g_i}(\boldsymbol x)$ is $i$-th generator's distribution, $p_{r_j}$ is distribution of region $r_j$. 


\comment{
\section{Applications}
\subsection{Semi supervised learning using complement generators}

In the context of semi-supervised learning with GANs, \cite{dai2017good} showed some needed property of the generator to achieve better semi-supervised learning performance. In their definition of preferred generator, they showed that the system needs a generator to generate samples in low density region to help for the training. Whereas in GAN setting an ideal generator's distribution $p_g(x)$ aims to match exactly to the data distribution $p_{data}(x)$. To improve classification tasks, it should be able to produce samples from the low density region of the data space. \cite{dai2017good} proposed some methods to enforce that constraint and observed that it effectively improves performance in practice. However, these improvements on top of the standard Improved GAN framework considerably increases the computational cost because they rely on an additional trained model providing a tractable likelihood of the generated samples from the generator $G$ .

% *** Some description about how this bad generator is related to complement of a set is missing ***

They define the idea of a complement generator for semi supervised learning. G is a function which maps latent representation $z \in Z$  to vectors in the image space $X$. $G: z\xrightarrow{}G(z)$. G define a probability distribution, $p_g(x)$, over the image space. Let $F_k$ be a subset of the $X$ such that $F_k=\{x:p_g >k\}$

An interesting property of our model is that it can learn easily complement of a sets in an unsupervised manner. More formally, if $A$ is a set of elements and $U$ is the universe, we can learn $A^c = \{x \in U | x\notin A\}$. We propose to evaluate if such a method to learn complement distribution could be an efficient way to shortcut the technical difficulties previously introduced and could be an efficient technique to produce samples from low density regions.

We propose to combine the training of a complement generator trained using the method proposed in this paper and a standard $K+1$ classifier for semi-supervised learning. The classifier is added on top of the GAN and do not interact with the rest of the system. However, the classifier perceives generated samples from the generator of the VennGAN which must ideally produce samples from the subsets $F_k^c$. In the next subsection, we propose experiments to test the following assertions:
\begin{enumerate}
\item VennGAN can learn the complement set $F_k^c$ of a complex distribution.
\item The complement generator improves the training of a semi-supervised $K+1$ classifier as demonstrated by \cite{dai2017good}.
\end{enumerate}
 
\subsubsection{Study on synthetic data}

We first show some examples of complement distribution in Figure \ref{fig_complement}. We have used ``v3'' type venn diagram with 2 sets where first distribution is a zero mean gaussian vector (blue region) and the second is the universe (orange region) which is anywhere inside $\left [ -1,1 \right ]\times \left [ -1,1 \right ]$.

\begin{figure}[h!]
	\centering
    \includegraphics[width=.9\linewidth]{figures/ssl/gauss_uni.png}
	\caption{Complement generator of a gaussian distribution in the paved space $\left [ -1.5,1 \right ]\times \left [ -1,1 \right ]$.}
	\label{fig_complement}
\end{figure}

We show here a study on a synthetic 2D dataset. We try to classify the two moons with only very few labeled samples and a large amount of unlabeled data. We train our VennGAN in addition to the $K+1$ classifier. 

\[L= L_{supervised} + L_{unsupervised}  \text{  ,where} \] 
\begin{align*} 
\label{ldis}
L_{supervised} &= - \mathbb{E}_{x,y \sim p_{data}(x,y)} \left[ \log{p_{f} (y|x,y<K+1)} \right]  \\
L_{unsupervised} &= -   \mathbb{E}_{x \sim p_{data}(x)} \left[ \log{[1- p_{f} (y=K+1|x)]} \right]  - \mathbb{E}_{x \sim g} \left[ \log {[p_{f} (y=K+1|x)]} \right] \\
\end{align*}

The experiment described in figure \ref{ssl} shows good results on different syntethic datasets.

\begin{figure}[h!]
\centering
\includegraphics[width=0.9\linewidth]{figures/ssl/moon2.png}\\
\includegraphics[width=0.9\linewidth]{figures/ssl/noisy_circle2.png}\\

\caption{Semi supervised learning on the two moons dataset using our \textit{bad} generator}
\label{ssl}
\end{figure}

\subsubsection{How to choose the universe in order to model the complement distribution?}

In our example, we chose naturally a paved space containing the set of clusters of data. This is not straight forward to choose this set in the case of other types of data. We conjecture that in the case of natural images, an additional dataset with different classes might be adapted.
%############################################################


\subsection{Improving GAN with Incremental Learning}
As VennGAN can see differences between the distributions a natural use case of it is, detecting missing modes in a pre-trained generator distribution. We have used ``v1'' type modeling with 2 distribution game, where the first distribution is CIFAR-10 and the second one is a pre-trained generator that mimics CIFAR-10 distribution. As initial step, we have trained a GAN on CIFAR-10, with DCGAN architecture (refer to the Appendix for detailed configuration). 

We have tried conditional generator to model this problem, however it fail to produce images different than previously generated ones (different conditions with the same noise produces similar images).

*** What about we show the benefit of this approach with a simpler dataset? ***
}

\begin{equation}\label{eq:data_distribution_mog}
    \begin{bmatrix}
        p_{data_1} \\
        p_{data_2} \\
        p_{data_3}
    \end{bmatrix}
    =
    \begin{bmatrix}
        \frac{\mathcal{N}(\mu_1 = \begin{bmatrix} -1 \\ -1\end{bmatrix},\Sigma)}{4} + \frac{\mathcal{N}(\mu_4,\Sigma)}{4} + \frac{\mathcal{N}(\mu_6,\Sigma)}{4} + \frac{\mathcal{N}(\mu_7,\Sigma)}{4} \\
        \frac{\mathcal{N}(\mu_2,\Sigma)}{4} + \frac{\mathcal{N}(\mu_5,\Sigma)}{4} + \frac{\mathcal{N}(\mu_6,\Sigma)}{4} + \frac{\mathcal{N}(\mu_7,\Sigma)}{4} \\
        \frac{\mathcal{N}(\mu_3,\Sigma)}{4} + \frac{\mathcal{N}(\mu_4,\Sigma)}{4} + \frac{\mathcal{N}(\mu_5,\Sigma)}{4} + \frac{\mathcal{N}(\mu_7,\Sigma)}{4}
    \end{bmatrix}
\end{equation}

where $\mathcal{N}(\mu,\Sigma)$ is a gaussian distribution with $\mu \in \mathbb{R}^{2}$  and $\Sigma \in \mathbb{R}^{2 \times 2}$, $\Sigma=0.1\times \mathbb{I}$, $\mu_1 = \begin{bmatrix} -1 \\ -1\end{bmatrix}$, $ \mu_2 = [0\ 1]^T$, $ \mu_3 = [1\ -1]^T$, $ \mu_4 = [0\ 0]^T$, $ \mu_5 = [0\ 0]^T$, $ \mu_6 = [0\ 0]^T$ and $ \mu_7 = [0\ 0]^T$, Fig.\ref{fig:gaussian_toy} (Right) 

\begin{equation}\label{eq:data_distribution_mog}
    \begin{bmatrix}
        p_{data_1} \\
        p_{data_2} \\
        p_{data_3}
    \end{bmatrix}
    =
    \begin{bmatrix}
        \frac{1}{4} & 0 & 0 & \frac{1}{4} & 0 & 0 & \frac{1}{4} & \frac{1}{4} \\
        0 & \frac{1}{4} & 0 & 0 & 0 & \frac{1}{4} & \frac{1}{4} & \frac{1}{4} \\
        0 & 0 & \frac{1}{4} & \frac{1}{4} & \frac{1}{4} & 0 & 0 & \frac{1}{4}
    \end{bmatrix}
    \begin{bmatrix}
        \mathcal{N}(\mu_1,\Sigma) \\
        \mathcal{N}(\mu_2,\Sigma) \\
        \mathcal{N}(\mu_3,\Sigma) \\
        \mathcal{N}(\mu_4,\Sigma) \\
        \mathcal{N}(\mu_5,\Sigma) \\
        \mathcal{N}(\mu_6,\Sigma) \\
        \mathcal{N}(\mu_7,\Sigma)
    \end{bmatrix}
\end{equation}

where $\mathcal{N}(\mu,\Sigma)$ is a gaussian distribution with $\mu \in \mathbb{R}^{2}$  and $\Sigma \in \mathbb{R}^{2 \times 2}$, $\Sigma=0.1\times \mathbb{I}$, Fig.\ref{fig:gaussian_toy} (Right)

In practice we observed leaking between the regions which is a direct result of equally weighting the regions (See Table~\ref{quantitative results} for experimental results of this phenomena). The leaking come in two different ways. In the first type low intersection regions includes some portion of high intersection regions such as leaking from 2,3-way intersection to no-intersection or from 3-way intersection to 2-way intersection. This happens when the weights of low intersection regions are higher than what it should be in true data distribution. That leads low intersection regions to help other regions in the union by taking some portions of them. The second type is reverse of the previous situation namely high-intersection regions represents some part of low-intersection regions. This happens when consensus loss is overwhelmed by large weights of high intersection regions which does not match to its correspondence in the true data distribution. In order to alleviate this issue we included an additional objective which aims to separate regions of the generator, one from another:

Think about a situation where $p_{data_1} = 0.4 p_{r_1} + 0.6 p_{r_2}$ and  $p_{data_2} = 0.5 p_{r_3} + 0.5 p_{r_2}$. This would correspond to:
\begin{equation}
    \begin{bmatrix}
        p_{data_1} \\
        p_{data_2}
    \end{bmatrix}
    =
    \begin{bmatrix}
        p_{g_1} \\
        p_{g_2}
    \end{bmatrix}
    =
    \begin{bmatrix}
        $0.4$ & $0.6$ & $0.0$ \\
        $0.0$ & $0.5$ & $0.5$
    \end{bmatrix}
    \begin{bmatrix}
        p_{r_1} \\
        p_{r_2} \\
        p_{r_3} \\
    \end{bmatrix}
\end{equation}

Maybe promote this as simple toy example where $p_{r_1}$, $p_{r_2}$, $p_{r_3}$ are gaussian distributions.

\textbf{Joint distribution GAN:} Different than conditional GAN, this one models marginal distribution together with conditional distribution. 


    \begin{bmatrix}
        p_{data_1} \\
        p_{data_2} \\
        \vdots \\
        p_{data_n}
    \end{bmatrix}
    =
    

%The method described above, converges to satisfactory results on various datasets when $\alpha$ values are properly tuned. However this is not an easy task as we don't know what should be the contributions of regions to model true data distributions correctly.
\begin{equation}
    \boldsymbol{p_{data}} = \boldsymbol{O} \boldsymbol{p_g}
\end{equation}

where $\boldsymbol{O} \in \mathbb{R}^{n \times n}$ is an identity matrix.


%By considering the relations between the distributions each of them can be modeled better. This method learns multiple distributions by exploiting relations between them. It also constrict generator and possibly improve the stability. For example, in $d_3$ type one set is superset of another. Since the common part of the distributions must be modeled with the subset. The generator should be able to place this part into its certain mode and spare the other mode for the rest which regularize its learning by restriction. In this way with $d_3$ we can learn image transformations however we spare detailed examination of this for the future work.

%GAN has been used in interesting application, mainly image transformations which maps one distributions into another one in a semantically meaningful way \cite{DBLP:journals/corr/IsolaZZE16,DBLP:journals/corr/ReedAYLSL16, DBLP:journals/corr/LedigTHCATTWS16}. This corresponds to learning a conditional distribution. Another application is learning joint distribution from marginal distributions \cite{DBLP:journals/corr/0001T16}. Even though these applications utilize multiple distributions, they do not explicitly learn commonalities and differences between the distributions. 

%Spectral normalization is used both in discriminator \cite{spectral_norm} and generator \cite{sagan}

